Modeling Terms by Graphs with Structure Constraints (Two Illustrations)

In the talk at the workshop my aim was to demonstrate the usefulness of graph techniques for tackling problems that have been studied predominantly as problems on the term level: increasing sharing in functional programs, and addressing questions about Milner's process semantics for regular expressions. For both situations an approach that is based on modeling terms by graphs with structure constraints has turned out to be fruitful. In this extended abstract I describe the underlying problems, give references, provide examples, indicate the chosen approaches, and compare the initial situations as well as the results that have been obtained, and some results that are being developed at present.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{M. Fern\'andez and I. Mackie (Eds.): TERMGRAPH 2018.\\
EPTCS 288, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.288.1}{10.4204/EPTCS.288.1}}
\pdfoutput=1


==> figs/L0-ldfa.tex <==
\begin{pgfonlayer}{graph}
%
%
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw,thick,scale=1,minimum size=0.4cm,inner sep=0pt}] at (7.1,-2) {
  & & \node[double](root-dfa-3){}; \\
  & & \node[double](0-dfa-3){}; \\ 
  & & \node[double](00-dfa-3){}; \\
  & \node[double](000-dfa-3){}; \\
  \node[double](0000-dfa-3){}; & & \node[double](helper1-dfa-3)[draw=none]{}; & & & \node[double](001){};\\   
  & & \node(helper2-dfa-3)[draw=none]{}; & & & \node[double](0010){};\\
}; 
\path (0000-dfa-3) ++ (0.75cm,-1.5cm) node[circle,draw,thick,scale=1,minimum size=0.4cm,inner sep=0pt](dummy){};    
% \\
%   & \node[yshift=0.35cm,xshift=-0.25cm](dummy){};\\

\draw[->,thick,chocolate,>=latex] ($(root-dfa-3.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-dfa-3.north) + (0pt,1pt)$);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-dfa-3) to node{\scriptsize \mbox{}\hspace*{-2.75ex}$\lambda$} (0-dfa-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-dfa-3) to node{\scriptsize \mbox{}\hspace*{-2.75ex}$\lambda$} (00-dfa-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-dfa-3) to node[near start]{\scriptsize \mbox{}\hspace*{-4ex}$@_0$} (000-dfa-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-dfa-3) to node[near start]{\scriptsize \mbox{}\hspace*{-4ex}$@_0$} (0000-dfa-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-dfa-3) to node[right]{\scriptsize $@_1$} (001);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001) to [right]node{\scriptsize $S_0$} (0010);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-dfa-3) to[out=-50,in=50,distance=1.75cm] node[above right]{\scriptsize $@_1$} (00-dfa-3); 
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0000-dfa-3) -- +(-1cm,0cm) |- node[below left]{\scriptsize $0$} (0-dfa-3.west);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001) -- ($ (helper1-dfa-3) + (2.65cm,0cm) $)  %($ (helper1-dfa-3) + (1.1cm,0cm) $)
               -- node[left]{\scriptsize $S_1$} ($ (0-dfa-3) + (2.65cm,0cm) $)        %($ (0-dfa-3) + (1.1cm,0cm) $)
               -- (0-dfa-3);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0010)  -- ($ (helper2-dfa-3) + (3.2cm,0cm) $)
                 -- node[right]{\scriptsize $0$} ($ (root-dfa-3) + (3.2cm,0cm) $)
                 -- (root-dfa-3);                    

\draw[->, bend right=80,distance=2.5cm,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-dfa-3) to[very near start] node{\scriptsize $0, @_{0/1}, S_{0/1}\hspace*{15ex}\mbox{}$} (dummy);
\draw[->, bend right=60,distance=2.25cm,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-dfa-3) to[very near start] node{\scriptsize $0, @_{0/1}, S_{0/1}\hspace*{4.75ex}\mbox{}$} (dummy);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-dfa-3) to[near start] node{\hspace*{7ex}\scriptsize $\lambda, 0, S_{0/1}$\mbox{}} (dummy);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-dfa-3) to[near start] node{\scriptsize $\lambda, 0, S_{0/1}$} (dummy);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0000-dfa-3) to[near start] node{\scriptsize $\lambda, @_{0/1}, S_{0/1}$} (dummy);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001) to[near start] node{\scriptsize $\lambda$, $0$, $@_{0/1}$\hspace*{12ex}\mbox{}} (dummy);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0010) to node{\scriptsize \mbox{}\hspace*{20ex}$\lambda$, $@_{0/1}$, $S_{0/1}$} (dummy);
 
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](dummy) to[out=270,in=180,distance=1.25cm] node[left]{\scriptsize $\lambda$, $0$, $@_{0/1}$, $\snlvarsucc_{0/1}$} (dummy);                   
%
% 
\end{pgfonlayer}


\begin{pgfonlayer}{caption}
  \path[draw=none] (root-dfa-3) -- ($ (root-dfa-3) + (0.25cm,-5.2cm) $) node{\emph{$\lambda$-DFA}};
\end{pgfonlayer}


\begin{pgfonlayer}{boundingbox}
  \path[thick,dotted,%draw,
                     use as bounding box]
         ($ (root-dfa-3.north) + (-3.5cm,0.5cm) $)
      -- ($ (root-dfa-3.north) + (-3.5cm,-5.9cm) $)
      -- ($ (root-dfa-3.north) + (+3.5cm,-5.9cm) $)
      -- ($ (root-dfa-3.north) + (+3.5cm,0.5cm) $)
      -- ($ (root-dfa-3.north) + (-3.5cm,0.5cm) $);  
\end{pgfonlayer}




==> figs/L0-lhotg-1.tex <==
\begin{pgfonlayer}{graph}
  %
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={draw,thick,circle,scale=1,minimum size=0.4cm,inner sep=0pt,red,fill=white}
                                                          %{circle,draw,thick,fill=white,scale=1,minimum size=0.4cm,inner sep=0pt}]
                                                          ] at (9,5.6) % at (1.5,-0.5) 
                                                                    {
  & & \node(root-lhotg-1){$\sslabs$}; \\
  & & \node(0-lhotg-1){$\sslabs$}; \\ 
  & & \node(00-lhotg-1){$\sslapp$}; \\
  & \node(000-lhotg-1){$\sslapp$}; \\
  \node(0000-lhotg-1){$\snlvar$}; & & \node(helper1-lhotg-1)[fill=none,draw=none]{}; \\   
  & & \node(helper2-lhotg-1)[fill=none,draw=none]{}; & & & & & \node(001){$\snlvar$};\\
};  
% \draw[<-,very thick,>=latex](root-lhotg-1.north) -- ++ (90:0.35cm);
\draw[->,thick,chocolate,>=latex] ($(root-lhotg-1.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-lhotg-1.north) + (0pt,1pt)$);
\draw[->,thick,red,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-lhotg-1) to (0-lhotg-1);
\draw[->,thick,red,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-lhotg-1) to (00-lhotg-1);
\draw[->,thick,red,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-lhotg-1) to (000-lhotg-1);
\draw[->,thick,red,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-lhotg-1) to (0000-lhotg-1);
\draw[->,thick,red,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-lhotg-1) to (001);
\draw[->,thick,red,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
    postaction={decorate}](000-lhotg-1) to[out=-50,in=50,distance=1.75cm] 
                  (00-lhotg-1);                   
%
\draw[->,thick,mediumblue,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0000-lhotg-1) -- ($ (helper1-lhotg-1) + (2.65cm,0cm) $)  %($ (helper1-lhotg-1) + (1.1cm,0cm) $)
                -- ($ (0-lhotg-1) + (2.65cm,0cm) $)        %($ (0-lhotg-1) + (1.1cm,0cm) $)
                -- (0-lhotg-1); 
% \draw[-,dashed](0-lhotg-1) -- ($ (0-lhotg-1)       + (-2.25cm,0cm) $)
%                    -- ($ (helper1-lhotg-1) + (-2.25cm,0cm) $)
%                    -- (0000-lhotg-1);                
%                                                
\draw[->,thick,mediumblue,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001) -- ($ (helper2-lhotg-1) + (3.2cm,0cm) $)
                     -- ($ (root-lhotg-1) + (3.2cm,0cm) $)
                     -- (root-lhotg-1);
% \draw[-,dashed](root-lhotg-1) -- ($ (root-lhotg-1) + (-2.8cm,0cm) $)
%                       -- ($ (helper2-lhotg-1) + (-2.8cm,0cm) $)
%                       -- (001);
\end{pgfonlayer}
%
% 
% 
\begin{pgfonlayer}{innerscope}    
  \draw[draw=none,fill=grey!27]
    (0000-lhotg-1) -- ($ (helper1-lhotg-1) + (2.65cm,0cm) $)  %($ (helper1-lhotg-1) + (1.1cm,0cm) $)
           -- ($ (0-lhotg-1)       + (2.65cm,0cm) $)        %($ (0-lhotg-1) + (1.1cm,0cm) $)\
           -- ($ (0-lhotg-1)       + (-2.65cm,0cm) $)
           -- ($ (helper1-lhotg-1) + (-2.65cm,0cm) $)
           -- (0000-lhotg-1);           
\end{pgfonlayer}{innerscope}
                                  

\begin{pgfonlayer}{outerscope}                                 
  \draw[draw=none,fill=grey!12]
    (001) -- ($ (helper2-lhotg-1) + (3.2cm,0cm) $)
          -- ($ (root-lhotg-1)    + (3.2cm,0cm) $)
          -- ($ (root-lhotg-1)    + (-3.2cm,0cm) $)
          -- ($ (helper2-lhotg-1) + (-3.2cm,0cm) $)
          -- (001);
\end{pgfonlayer}                                        

\begin{pgfonlayer}{caption}
  \path[draw=none] (root-lhotg-1) -- ($ (root-lhotg-1) + (0cm,-4.6cm) $) node{\textcolor{red}{first-order term graph}};
  \path[draw=none] (root-lhotg-1) -- ($ (root-lhotg-1) + (0cm,-5.1cm) $) node{{with \mediumblue{binding backlinks} (+ scope sets)}};
\end{pgfonlayer}


\begin{pgfonlayer}{background}
\path[thick,dotted,%draw,
                   use as bounding box]
       ($ (root-lhotg-1.north) + (-3.5cm,0.5cm) $)
    -- ($ (root-lhotg-1.north) + (-3.5cm,-5.6cm) $)
    -- ($ (root-lhotg-1.north) + (+3.5cm,-5.6cm) $)
    -- ($ (root-lhotg-1.north) + (+3.5cm,0.5cm) $)
    -- ($ (root-lhotg-1.north) + (-3.5cm,0.5cm) $);  
\end{pgfonlayer}{background}                         



==> figs/L0-lhotg-3.tex <==
\begin{pgfonlayer}{graph}
%  
%  
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw,thick,fill=white,scale=1,minimum size=0.4cm,inner sep=0pt}] at (7.5,11) % at (0,4.5) 
                                                                                                                                                            {
  & & \node(root-lhotg-3){$\sslabs$}; \\
  & & \node(0-lhotg-3){$\sslabs$}; \\ 
  & & \node(00-lhotg-3){$\sslapp$}; \\
  & \node(000-lhotg-3){$\sslapp$}; \\
  \node(0000-lhotg-3){$\snlvar$}; & & \node(helper1)[fill=none,draw=none]{};\\   
  & & \node(helper2)[fill=none,draw=none]{}; & & & & & \node(001){$\snlvar$};\\
}; 
\draw[->,chocolate,thick,>=latex] ($(root-lhotg-3.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-lhotg-3.north) + (0pt,1pt)$);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-lhotg-3) to (0-lhotg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-lhotg-3) to (00-lhotg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-lhotg-3) to (000-lhotg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-lhotg-3) to (0000-lhotg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-lhotg-3) to (001);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-lhotg-3) to[out=-50,in=50,distance=1.75cm] 
                  (00-lhotg-3); 
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0000-lhotg-3) -- ($ (helper1) + (2.65cm,0cm) $)  %($ (helper1) + (1.1cm,0cm) $)
                -- ($ (0-lhotg-3) + (2.65cm,0cm) $)        %($ (0-lhotg-3) + (1.1cm,0cm) $)
                -- (0-lhotg-3);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001)  -- ($ (helper2) + (3.2cm,0cm) $)
                -- ($ (root-lhotg-3) + (3.2cm,0cm) $)
                -- (root-lhotg-3);  
%
%                                   
\end{pgfonlayer}                  
%
% 
\begin{pgfonlayer}{innerscope}    
  \draw[draw=none,fill=grey!27]
    (0000-lhotg-3) -- ($ (helper1) + (2.65cm,0cm) $)  %($ (helper1) + (1.1cm,0cm) $)
           -- ($ (0-lhotg-3)       + (2.65cm,0cm) $)        %($ (0-lhotg-3) + (1.1cm,0cm) $)\
           -- ($ (0-lhotg-3)       + (-2.65cm,0cm) $)
           -- ($ (helper1) + (-2.65cm,0cm) $)
           -- (0000-lhotg-3);           
\end{pgfonlayer}{innerscope}
%                                  
%
\begin{pgfonlayer}{outerscope}                                 
  \draw[draw=none,fill=grey!12]
    (001) -- ($ (helper2) + (3.2cm,0cm) $)
          -- ($ (root-lhotg-3)    + (3.2cm,0cm) $)
          -- ($ (root-lhotg-3)    + (-3.2cm,0cm) $)
          -- ($ (helper2) + (-3.2cm,0cm) $)
          -- (001);
\end{pgfonlayer}                                        


\begin{pgfonlayer}{caption}
  \path[draw=none] (root-lhotg-3) -- ($ (root-lhotg-3) + (0cm,-4.6cm) $) node{{first-order term graph with binding backlinks}};
  \path[draw=none] (root-lhotg-3) -- ($ (root-lhotg-3) + (0cm,-5.1cm) $) node{{(+ scope sets)}};
\end{pgfonlayer}  

                          
\begin{pgfonlayer}{boundingbox}                     
\path[thick,dotted,%draw,
                   use as bounding box]
       ($ (root-lhotg-3.north) + (-3.5cm,0.5cm) $)
    -- ($ (root-lhotg-3.north) + (-3.5cm,-5.6cm) $)
    -- ($ (root-lhotg-3.north) + (+3.5cm,-5.6cm) $)
    -- ($ (root-lhotg-3.north) + (+3.5cm,0.5cm) $)
    -- ($ (root-lhotg-3.north) + (-3.5cm,0.5cm) $);
\end{pgfonlayer}

==> figs/L0-lhotg-3a.tex <==
\begin{pgfonlayer}{graph}
%  
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw,thick,fill=white,scale=1,minimum size=0.4cm,inner sep=0pt}] at (1.5,-1) { % at (9,-0.5) {}
  & & \node(root-lhotg-3a){$\sslabs$}; \\
  & & \node(0-root-lhotg-3a){$\sslabs$}; \\ 
  & & \node(00-root-lhotg-3a){$\sslapp$}; \\
  & \node(000-root-lhotg-3a){$\sslapp$}; \\
  \node(0000-root-lhotg-3a){$\snlvar$}; & & \node(helper1)[fill=none,draw=none]{};\\   
  & & \node(helper2)[fill=none,draw=none]{}; & & & & & \node(001-root-lhotg-3a){$\snlvar$};\\
}; 
\draw[->,thick,chocolate,>=latex] ($(root-lhotg-3a.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-lhotg-3a.north) + (0pt,1pt)$);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-lhotg-3a) to (0-root-lhotg-3a);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-root-lhotg-3a) to (00-root-lhotg-3a);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-root-lhotg-3a) to (000-root-lhotg-3a);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-root-lhotg-3a) to (0000-root-lhotg-3a);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-root-lhotg-3a) to (001-root-lhotg-3a);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-root-lhotg-3a) to[out=-50,in=50,distance=1.75cm] 
                  (00-root-lhotg-3a); 
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0000-root-lhotg-3a) -- ($ (helper1) + (2.65cm,0cm) $)  %($ (helper1) + (1.1cm,0cm) $)
                -- ($ (0-root-lhotg-3a) + (2.65cm,0cm) $)        %($ (0-root-lhotg-3a) + (1.1cm,0cm) $)
                -- (0-root-lhotg-3a);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001-root-lhotg-3a)  -- ($ (helper2) + (3.2cm,0cm) $)
                -- ($ (root-lhotg-3a) + (3.2cm,0cm) $)
                -- (root-lhotg-3a);   
%                                        
\end{pgfonlayer}                  


\begin{pgfonlayer}{innerscope}    
  \draw[draw=none,fill=red!27]
    (0000-root-lhotg-3a) -- ($ (helper1) + (2.65cm,0cm) $)  %($ (helper1) + (1.1cm,0cm) $)
           -- ($ (0-root-lhotg-3a)       + (2.65cm,0cm) $)        %($ (0-root-lhotg-3a) + (1.1cm,0cm) $)\
           -- ($ (0-root-lhotg-3a)       + (-2.65cm,0cm) $)
           -- ($ (helper1) + (-2.65cm,0cm) $)
           -- (0000-root-lhotg-3a);           
\end{pgfonlayer}{innerscope} 


\begin{pgfonlayer}{outerscope}                                 
  \draw[draw=none,fill=red!12]
    (001-root-lhotg-3a) -- ($ (helper2) + (3.2cm,0cm) $)
          -- ($ (root-lhotg-3a)    + (3.2cm,0cm) $)
          -- ($ (root-lhotg-3a)    + (-3.2cm,0cm) $)
          -- ($ (helper2) + (-3.2cm,0cm) $)
          -- (001-root-lhotg-3a);
\end{pgfonlayer}                                        

            
\begin{pgfonlayer}{caption}
  \path[draw=none] (root-lhotg-3a) -- ($ (root-lhotg-3a) + (0cm,-4.7cm) $) node{\emph{$\lambda$-higher-order term graph}, version 1:};
  \path[draw=none] (root-lhotg-3a) -- ($ (root-lhotg-3a) + (0cm,-5.2cm) $) node{term graph {with \textcolor{red}{scope sets}}};
  \path[draw=none] (root-lhotg-3a) -- ($ (root-lhotg-3a) + (0cm,-5.6cm) $) node{{as structure constraints}};
\end{pgfonlayer}


\begin{pgfonlayer}{background}
\path[thick,dotted,%draw,
                   use as bounding box]
       ($ (root-lhotg-3a.north) + (-3.5cm,0.5cm) $)
    -- ($ (root-lhotg-3a.north) + (-3.5cm,-6.1cm) $)
    -- ($ (root-lhotg-3a.north) + (+3.5cm,-6.1cm) $)
    -- ($ (root-lhotg-3a.north) + (+3.5cm,0.5cm) $)
    -- ($ (root-lhotg-3a.north) + (-3.5cm,0.5cm) $);  
\end{pgfonlayer}{background} 

==> figs/L0-lhotg-4.tex <==
\begin{pgfonlayer}{graph}
%  
%  
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw,thick,fill=white,scale=1,minimum size=0.4cm,inner sep=0pt}] at (0,11) % at (7.5,11) 
                                                                                                                                                          {
  & & \node(root-lhotg-4){$\sslabs$}; \\
  & & \node(0-lhotg-4){$\sslabs$}; \\ 
  & & \node(00-lhotg-4){$\sslapp$}; \\
  & \node(000-lhotg-4){$\sslapp$}; \\
  \node(0000-lhotg-4){$\snlvar$}; & & \node(helper1-lhotg-4)[fill=none,draw=none]{};\\   
  & & \node(helper2-lhotg-4)[fill=none,draw=none]{}; & & & & & \node(001-lhotg-4){$\snlvar$};\\
}; 
\draw[->,chocolate,thick,>=latex] ($(root-lhotg-4.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-lhotg-4.north) + (0pt,1pt)$);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-lhotg-4) to (0-lhotg-4);
\addvertname{root-lhotg-4}{\averti{0}}
\addvertprefix{root-lhotg-4}{\niks}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-lhotg-4) to (00-lhotg-4);
\addvertname{0-lhotg-4}{\averti{1}}
\addvertprefix{0-lhotg-4}{\averti{0}}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-lhotg-4) to (000-lhotg-4);
\addvertprefix{00-lhotg-4}{\averti{0}\averti{1}}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-lhotg-4) to (0000-lhotg-4);
\addvertprefix{000-lhotg-4}{\averti{0}\averti{1}}
\addvertprefix{0000-lhotg-4}{\averti{0}\averti{1}}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-lhotg-4) to (001-lhotg-4);
\addvertprefixpos{001-lhotg-4}{\averti{0}}{-0.4ex}{-0.75ex}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-lhotg-4) to[out=-50,in=50,distance=1.75cm] 
                  (00-lhotg-4); 
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0000-lhotg-4) -- ($ (helper1-lhotg-4) + (2.65cm,0cm) $)  %($ (helper1-lhotg-4) + (1.1cm,0cm) $)
                -- ($ (0-lhotg-4) + (2.65cm,0cm) $)        %($ (0-lhotg-4) + (1.1cm,0cm) $)
                -- (0-lhotg-4);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001-lhotg-4)  -- ($ (helper2-lhotg-4) + (3.2cm,0cm) $)
                -- ($ (root-lhotg-4) + (3.2cm,0cm) $)
                -- (root-lhotg-4);  
%
%                                   
\end{pgfonlayer}                  
%
% 
% 
\begin{pgfonlayer}{innerscope}    
  \draw[draw=none,fill=none]
    (0000-lhotg-4) -- ($ (helper1-lhotg-4) + (2.65cm,0cm) $)  %($ (helper1-lhotg-4) + (1.1cm,0cm) $)
           -- ($ (0-lhotg-4)       + (2.65cm,0cm) $)        %($ (0-lhotg-4) + (1.1cm,0cm) $)\
           -- ($ (0-lhotg-4)       + (-2.6cm,0cm) $)
           -- ($ (helper1-lhotg-4) + (-2.6cm,0cm) $)
           -- (0000-lhotg-4);           
\end{pgfonlayer}{innerscope}
%                                  
%
\begin{pgfonlayer}{outerscope}                                 
  \draw[draw=none,fill=none]
    (001-lhotg-4) -- ($ (helper2-lhotg-4) + (3.2cm,0cm) $)
          -- ($ (root-lhotg-4)    + (3.2cm,0cm) $)
          -- ($ (root-lhotg-4)    + (-3.25cm,0cm) $)
          -- ($ (helper2-lhotg-4) + (-3.25cm,0cm) $)
          -- (001-lhotg-4);
\end{pgfonlayer}                                        


\begin{pgfonlayer}{caption}
  \path[draw=none] (root-lhotg-4) -- ($ (root-lhotg-4) + (0cm,-4.6cm) $) node{$\lambda$\nb-higher-order-term-graph};
  \path[draw=none] (root-lhotg-4) -- ($ (root-lhotg-4) + (0cm,-5.1cm) $) node{{with {abstraction prefix function}}};
\end{pgfonlayer}


\begin{pgfonlayer}{background}
  \path[thick,dotted,%draw,
                     use as bounding box]
         ($ (root-lhotg-4.north) + (-3.5cm,0.5cm) $)
      -- ($ (root-lhotg-4.north) + (-3.5cm,-5.6cm) $)
      -- ($ (root-lhotg-4.north) + (+3.5cm,-5.6cm) $)
      -- ($ (root-lhotg-4.north) + (+3.5cm,0.5cm) $)
      -- ($ (root-lhotg-4.north) + (-3.5cm,0.5cm) $);  
\end{pgfonlayer}{background} 

==> figs/L0-lhotg-4a.tex <==
\begin{pgfonlayer}{graph}
%  
%  
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw,thick,fill=white,scale=1,minimum size=0.4cm,inner sep=0pt}] at (9,-1) % at (0,11) 
                                                                                                                                                            {
  & & \node(root-lhotg-4a){$\sslabs$}; \\
  & & \node(0-lhotg-4a){$\sslabs$}; \\ 
  & & \node(00-lhotg-4a){$\sslapp$}; \\
  & \node(000-lhotg-4a){$\sslapp$}; \\
  \node(0000-lhotg-4a){$\snlvar$}; & & \node(helper1-lhotg-4a)[fill=none,draw=none]{};\\   
  & & \node(helper2)[fill=none,draw=none]{}; & & & & & \node(001-lhotg-4a){$\snlvar$};\\
}; 
\draw[->,thick,chocolate,>=latex] ($(root-lhotg-4a.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-lhotg-4a.north) + (0pt,1pt)$);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-lhotg-4a) to (0-lhotg-4a);
\addvertnamedarkcyan{root-lhotg-4a}{\averti{0}}
\addvertprefixalert{root-lhotg-4a}{\niks}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-lhotg-4a) to (00-lhotg-4a);
\addvertnamedarkcyan{0-lhotg-4a}{\averti{1}}
\addvertprefixalert{0-lhotg-4a}{\averti{0}}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-lhotg-4a) to (000-lhotg-4a);
\addvertprefixalert{00-lhotg-4a}{\averti{0}\averti{1}}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-lhotg-4a) to (0000-lhotg-4a);
\addvertprefixalert{000-lhotg-4a}{\averti{0}\averti{1}}
\addvertprefixalert{0000-lhotg-4a}{\averti{0}\averti{1}}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-lhotg-4a) to (001-lhotg-4a);
\addvertprefixposalert{001-lhotg-4a}{\averti{0}}{-0.4ex}{-0.75ex}
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-lhotg-4a) to[out=-50,in=50,distance=1.75cm] 
                  (00-lhotg-4a); 
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0000-lhotg-4a) -- ($ (helper1-lhotg-4a) + (2.65cm,0cm) $)  %($ (helper1-lhotg-4a) + (1.1cm,0cm) $)
                -- ($ (0-lhotg-4a) + (2.65cm,0cm) $)        %($ (0-lhotg-4a) + (1.1cm,0cm) $)
                -- (0-lhotg-4a);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001-lhotg-4a)  -- ($ (helper2) + (3.2cm,0cm) $)
                -- ($ (root-lhotg-4a) + (3.2cm,0cm) $)
                -- (root-lhotg-4a);  
%
%                                   
\end{pgfonlayer}                  
%
% 
% 
\begin{pgfonlayer}{innerscope}    
  \draw[draw=none,fill=none]
    (0000-lhotg-4a) -- ($ (helper1-lhotg-4a) + (2.65cm,0cm) $)  %($ (helper1-lhotg-4a) + (1.1cm,0cm) $)
           -- ($ (0-lhotg-4a)       + (2.65cm,0cm) $)        %($ (0-lhotg-4a) + (1.1cm,0cm) $)\
           -- ($ (0-lhotg-4a)       + (-2.6cm,0cm) $)
           -- ($ (helper1-lhotg-4a) + (-2.6cm,0cm) $)
           -- (0000-lhotg-4a);           
\end{pgfonlayer}{innerscope}
%                                  
%
\begin{pgfonlayer}{outerscope}                                 
  \draw[draw=none,fill=none]
    (001-lhotg-4a) -- ($ (helper2) + (3.2cm,0cm) $)
          -- ($ (root-lhotg-4a)    + (3.2cm,0cm) $)
          -- ($ (root-lhotg-4a)    + (-3.25cm,0cm) $)
          -- ($ (helper2) + (-3.25cm,0cm) $)
          -- (001-lhotg-4a);
\end{pgfonlayer}                                        

                          
\begin{pgfonlayer}{caption}
  \path[draw=none] (root-lhotg-3a) -- ($ (root-lhotg-4a) + (0cm,-4.7cm) $) node{\emph{$\lambda$-higher-order term graph}, version~2:};
  \path[draw=none] (root-lhotg-4a) -- ($ (root-lhotg-4a) + (0cm,-5.2cm) $) node{term graph {with \textcolor{red}{abstraction prefix function}}};
  \path[draw=none] (root-lhotg-4a) -- ($ (root-lhotg-4a) + (0cm,-5.6cm) $) node{{as structure constraint}};
\end{pgfonlayer}


\begin{pgfonlayer}{background}
  \path[thick,dotted,%draw,
                     use as bounding box]
         ($ (root-lhotg-4a.north) + (-3.5cm,0.5cm) $)
      -- ($ (root-lhotg-4a.north) + (-3.5cm,-6.1cm) $)
      -- ($ (root-lhotg-4a.north) + (+3.5cm,-6.1cm) $)
      -- ($ (root-lhotg-4a.north) + (+3.5cm,0.5cm) $)
      -- ($ (root-lhotg-4a.north) + (-3.5cm,0.5cm) $);  
\end{pgfonlayer}{background} 

==> figs/L0-lnfa-2.tex <==
\begin{pgfonlayer}{graph}
%
%
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw,thick,scale=1,minimum size=0.4cm,inner sep=0pt}] at (-0.38,-2) {
  & & \node[double](root-lnfa-2){}; \\
  & & \node[double](0-lnfa-2){}; \\ 
  & & \node[double](00-lnfa-2){}; \\
  & \node[double](000-lnfa-2){}; \\
  \node[double](0000-lnfa-2){}; & & \node(helper1)[double,draw=none]{}; & & & \node[double](001-lnfa-2){};\\   
  & & \node[double](helper2)[draw=none]{}; & & & \node[double](0010-lnfa-2){};\\
};    
\draw[->,thick,chocolate,>=latex] ($(root-lnfa-2.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-lnfa-2.north) + (0pt,1pt)$);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (root-lnfa-2) to node[left]{$\scriptstyle \lambda$} (0-lnfa-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (0-lnfa-2) to node[left]{$\scriptstyle \lambda$} (00-lnfa-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (00-lnfa-2) to node[near start,left]{$\scriptstyle @_0$} (000-lnfa-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (000-lnfa-2) to node[near start,left]{$\scriptstyle @_0$} (0000-lnfa-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (00-lnfa-2) to node[right]{$\scriptstyle @_1$} (001-lnfa-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (001-lnfa-2) to [right]node{$\scriptstyle S_0$} (0010-lnfa-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (000-lnfa-2) to[out=-50,in=50,distance=1.75cm] node[above right]{$\scriptstyle @_1$} (00-lnfa-2); 
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (0000-lnfa-2) -- +(-1cm,0cm) |- node[below left]{$\scriptstyle 0$} (0-lnfa-2.west);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (001-lnfa-2) -- ($ (helper1) + (2.65cm,0cm) $)  %($ (helper1) + (1.1cm,0cm) $)
               -- node[left]{$\scriptstyle S_1$} ($ (0-lnfa-2) + (2.65cm,0cm) $)        %($ (0-lnfa-2) + (1.1cm,0cm) $)
               -- (0-lnfa-2);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}]
       (0010-lnfa-2)  -- ($ (helper2) + (3.2cm,0cm) $)
                 -- node[right]{$\scriptstyle 0$} ($ (root-lnfa-2) + (3.2cm,0cm) $)
                 -- (root-lnfa-2); 
%
%                                     
\end{pgfonlayer}                  
        
                  
\begin{pgfonlayer}{caption}
  \path[draw=none] (root-lnfa-2) -- ($ (root-lnfa-2) + (0cm,-5.2cm) $) node{\emph{incomplete $\lambda$-DFA}};
\end{pgfonlayer}


\begin{pgfonlayer}{boundingbox}
  \path[thick,dotted,%draw,
                     use as bounding box]
         ($ (root-lnfa-2.north) + (-3.5cm,0.5cm) $)
      -- ($ (root-lnfa-2.north) + (-3.5cm,-5.9cm) $)
      -- ($ (root-lnfa-2.north) + (+3.5cm,-5.9cm) $)
      -- ($ (root-lnfa-2.north) + (+3.5cm,0.5cm) $)
      -- ($ (root-lnfa-2.north) + (-3.5cm,0.5cm) $);  
\end{pgfonlayer}

==> figs/L0-ltg-1.tex <==
\begin{pgfonlayer}{graph}
%  
%  
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,fill=white,draw,thick,scale=1,minimum size=0.4cm,inner sep=0pt}] at (-0.4,4.5) % at (7.1,4.5) 
                                                                                                                                                           {
  & & \node(root-ltg-3){$\sslabs$}; \\
  & & \node(0-ltg-3){$\sslabs$}; \\ 
  & & \node(00-ltg-3){$\sslapp$}; \\
  & \node(000-ltg-3){$\sslapp$}; \\
  \node(0000-ltg-3){$\snlvar$}; & & \node(helper1-ltg-1)[draw=none,fill=none]{}; & & & \node(001-ltg-3)[draw,thick,circle,scale=1,minimum size=0.4cm,inner sep=0pt,red,fill=white]{${\snlvarsucc}$};\\   
  & & \node(helper2-ltg-1)[draw=none,fill=none]{}; & & & \node(0010-ltg-3){$\snlvar$};\\
};    
\draw[->,thick,chocolate,>=latex] ($(root-ltg-3.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-ltg-3.north) + (0pt,1pt)$);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-ltg-3) to (0-ltg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-ltg-3) to (00-ltg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-ltg-3) to (000-ltg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-ltg-3) to (0000-ltg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-ltg-3) to (001-ltg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001-ltg-3) to (0010-ltg-3);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-ltg-3) to[out=-50,in=50,distance=1.75cm] 
                  (00-ltg-3); 
\draw[-](0000-ltg-3) -- ($ (001-ltg-3.west) + (-2pt,0pt) $);                  
\draw[->,red,thick,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
               postaction={decorate}](001-ltg-3) -- ($ (helper1-ltg-1) + (2.65cm,0cm) $)  %($ (helper1-ltg-1) + (1.1cm,0cm) $)
               -- ($ (0-ltg-3) + (2.65cm,0cm) $)        %($ (0-ltg-3) + (1.1cm,0cm) $)
               -- (0-ltg-3);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0010-ltg-3)  -- ($ (helper2-ltg-1) + (3.2cm,0cm) $)
                 -- ($ (root-ltg-3) + (3.2cm,0cm) $)
                 -- (root-ltg-3); 
%
%                                     
\end{pgfonlayer}                  
%
% 
% 
\begin{pgfonlayer}{innerscope}    
  \draw[draw=none,fill=grey!27]
    (0000-ltg-3) -- ($ (helper1-ltg-1) + (2.65cm,0cm) $)  %($ (helper1-ltg-1) + (1.1cm,0cm) $)
           -- ($ (0-ltg-3)       + (2.65cm,0cm) $)        %($ (0-ltg-3) + (1.1cm,0cm) $)\
           -- ($ (0-ltg-3)       + (-2.65cm,0cm) $)
           -- ($ (helper1-ltg-1) + (-2.65cm,0cm) $)
           -- (0000-ltg-3);           
\end{pgfonlayer}{innerscope}
%                                  
%
\begin{pgfonlayer}{outerscope}                                 
  \draw[draw=none,fill=grey!12]
    (0010-ltg-3) -- ($ (helper2-ltg-1) + (3.2cm,0cm) $)
           -- ($ (root-ltg-3) + (3.2cm,0cm) $)
           -- ($ (root-ltg-3) + (-3.2cm,0cm) $)
           -- ($ (helper2-ltg-1) + (-3.2cm,0cm) $)
           -- (0010-ltg-3);
\end{pgfonlayer}


\begin{pgfonlayer}{caption}
  \path[draw=none] (root-ltg-3) -- ($ (root-ltg-3) + (0cm,-4.6cm) $) node{{first-order term graph with}};
  \path[draw=none] (root-ltg-3) -- ($ (root-ltg-3) + (0cm,-5.1cm) $) node{{\textcolor{red}{scope vertices with backlinks} (+ scope sets)}};
\end{pgfonlayer}  

                          
\begin{pgfonlayer}{boundingbox}                     
\path[thick,dotted,%draw,
                   use as bounding box]
       ($ (root-ltg-3.north) + (-3.5cm,0.5cm) $)
    -- ($ (root-ltg-3.north) + (-3.5cm,-5.6cm) $)
    -- ($ (root-ltg-3.north) + (+3.5cm,-5.6cm) $)
    -- ($ (root-ltg-3.north) + (+3.5cm,0.5cm) $)
    -- ($ (root-ltg-3.north) + (-3.5cm,0.5cm) $);
\end{pgfonlayer}

==> figs/L0-ltg-2.tex <==
\begin{pgfonlayer}{graph}
%
% 
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw,thick,scale=1,minimum size=0.4cm,inner sep=0pt}]  at (7.1,4.5) % at (-0.4,-4.35) 
                                                                                                                                      {
  & & \node(root-ltg-2){$\sslabs$}; \\
  & & \node(0-ltg-2){$\sslabs$}; \\ 
  & & \node(00-ltg-2){$\sslapp$}; \\
  & \node(000-ltg-2){$\sslapp$}; \\
  \node(0000-ltg-2){$\snlvar$}; & & \node(helper1-ltg-2)[draw=none]{}; & & & \node(001-ltg-2){$\snlvarsucc$};\\   
  & & \node(helper2-ltg-2)[draw=none]{}; & & & \node(0010-ltg-2){$\snlvar$};\\
};    
\draw[->,thick,chocolate,>=latex] ($(root-ltg-2.north) + (0pt,1pt) + (0pt,0.35cm)$) -- ($(root-ltg-2.north) + (0pt,1pt)$);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](root-ltg-2) to (0-ltg-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0-ltg-2) to (00-ltg-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-ltg-2) to (000-ltg-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-ltg-2) to (0000-ltg-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](00-ltg-2) to (001-ltg-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001-ltg-2) to (0010-ltg-2);
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](000-ltg-2) to[out=-50,in=50,distance=1.75cm] 
                  (00-ltg-2); 
\draw[-](0000-ltg-2) -- ($ (001-ltg-2.west) + (-2pt,0pt) $);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](001-ltg-2) -- ($ (helper1-ltg-2) + (2.65cm,0cm) $)  %($ (helper1-ltg-2) + (1.1cm,0cm) $)
               -- ($ (0-ltg-2) + (2.65cm,0cm) $)        %($ (0-ltg-2) + (1.1cm,0cm) $)
               -- (0-ltg-2);                  
\draw[->,decoration={markings,mark=at position 1 with {\arrow[thick]{>}}},
         postaction={decorate}](0010-ltg-2)  -- ($ (helper2-ltg-2) + (3.2cm,0cm) $)
                 -- ($ (root-ltg-2) + (3.2cm,0cm) $)
                 -- (root-ltg-2);                    
%
%                   
\end{pgfonlayer}  
  
    
\begin{pgfonlayer}{caption}
  \path[draw=none] (root-ltg-2) -- ($ (root-ltg-2) + (0cm,-4.6cm) $) node{\emph{$\lambda$\nb-term graph}: first-order term graph};
  \path[draw=none] (root-ltg-2) -- ($ (root-ltg-2) + (0cm,-5.1cm) $) node{with scope vertices with backlinks};
\end{pgfonlayer}  

                          
\begin{pgfonlayer}{boundingbox}                     
\path[thick,dotted,%draw,
                   use as bounding box]
       ($ (root-ltg-2.north) + (-3.5cm,0.5cm) $)
    -- ($ (root-ltg-2.north) + (-3.5cm,-5.6cm) $)
    -- ($ (root-ltg-2.north) + (+3.5cm,-5.6cm) $)
    -- ($ (root-ltg-2.north) + (+3.5cm,0.5cm) $)
    -- ($ (root-ltg-2.north) + (-3.5cm,0.5cm) $);
\end{pgfonlayer}

==> figs/L0-syntax-tree-0.tex <==
\begin{pgfonlayer}{graph}
%
%
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw=none,scale=1,minimum size=0.4cm,inner sep=0pt}] at (0.7,11.3) {
  & & \node(root-syntax-tree-0){$\slabs{\avar}$}; \\
  & & \node(0-syntax-tree-0){$\slabs{f}$}; \\ 
  & & \node(00-syntax-tree-0){$\sslapp$}; \\
  & \node(000-syntax-tree-0){$\sslapp$}; & & \node(001-syntax-tree-0){$\avar$}; \\
  \node(0000-syntax-tree-0){$f$}; & & \node[color=red](0001-syntax-tree-0){$r$};\\   
};    
\draw[-](root-syntax-tree-0) to (0-syntax-tree-0);
\draw[-](0-syntax-tree-0) to (00-syntax-tree-0);
\draw[-](00-syntax-tree-0) to (000-syntax-tree-0);
\addvertnameposalert{00-syntax-tree-0}{r}{-3ex}{2.3ex}
\draw[-](000-syntax-tree-0) to (0000-syntax-tree-0);
\draw[-](000-syntax-tree-0) to (0001-syntax-tree-0);
\draw[-](00-syntax-tree-0) to (001-syntax-tree-0);
%
% 
\end{pgfonlayer}


\begin{pgfonlayer}{caption}
  \path[draw=none] (root-syntax-tree-0) -- ($ (root-syntax-tree-0) + (0cm,-4.25cm) $) node{{syntax tree}};
\end{pgfonlayer}  
  
\begin{pgfonlayer}{boundingbox}  
  \path[thick,dotted,%draw,%,color=white
                     use as bounding box]
         ($ (root-syntax-tree-0.north) + (-3.5cm,0.15cm) $)
      -- ($ (root-syntax-tree-0.north) + (-3.5cm,-4.8cm) $)
      -- ($ (root-syntax-tree-0.north) + (+3.5cm,-4.8cm) $)
      -- ($ (root-syntax-tree-0.north) + (+3.5cm,0.15cm) $)
      -- ($ (root-syntax-tree-0.north) + (-3.5cm,0.15cm) $);
\end{pgfonlayer}    

==> figs/L0-syntax-tree-2.tex <==
\begin{pgfonlayer}{graph}
%
% 
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw=none,scale=1,minimum size=0.4cm,inner sep=0pt}] at (8.2,11.3) {
  & & \node(root-syntax-tree-2){$\slabs{\avar}$}; \\
  & & \node(0-syntax-tree-2){$\slabs{f}$}; \\ 
  & & \node(00-syntax-tree-2){$\sslapp$}; \\
  & \node(000-syntax-tree-2){$\sslapp$}; & & \node(001-syntax-tree-2){$\avar$}; \\
  \node(0000-syntax-tree-2){$f$}; \\   
};    
\draw[-](root-syntax-tree-2) to (0-syntax-tree-2);
\draw[-](0-syntax-tree-2) to (00-syntax-tree-2);
\draw[-](00-syntax-tree-2) to (000-syntax-tree-2);
\addvertnameposalert{00-syntax-tree-2}{r}{-3ex}{2.3ex}
%\addvertnameposalert{00}{r}{0.25ex}{1.25ex}
\draw[-](000-syntax-tree-2) to (0000-syntax-tree-2);
\draw[-](00-syntax-tree-2) to (001-syntax-tree-2);
\draw[->,thick,red]%,alert,decoration={markings,mark=at position 1 with {\arrow[very thick]{>}}},
         %postaction={decorate}]
     (000-syntax-tree-2) to[out=-50,in=50,distance=1.75cm] (00-syntax-tree-2); 
%
% 
\end{pgfonlayer}


\begin{pgfonlayer}{caption}
  \path[draw=none] (root-syntax-tree-2) -- ($ (root-syntax-tree-2) + (0cm,-4.25cm) $) node{{syntax tree with \textcolor{red}{recursive backlink}}};
\end{pgfonlayer}


\begin{pgfonlayer}{boundingbox}
  \path[thick,dotted,%draw,
                     use as bounding box]
         ($ (root-syntax-tree-2.north) + (-3.5cm,0.15cm) $)
      -- ($ (root-syntax-tree-2.north) + (-3.5cm,-4.8cm) $)
      -- ($ (root-syntax-tree-2.north) + (+3.5cm,-4.8cm) $)
      -- ($ (root-syntax-tree-2.north) + (+3.5cm,0.15cm) $)
      -- ($ (root-syntax-tree-2.north) + (-3.5cm,0.15cm) $);
\end{pgfonlayer}    

==> figs/L0-syntax-tree-5.tex <==
\begin{pgfonlayer}{graph}
%  
% 
\matrix[anchor=north,row sep=0.35cm,column sep=0.4cm,every node/.style={circle,draw=none,scale=1,minimum size=0.4cm,inner sep=0pt}] at (1.5,5.75) %at (9,6) 
                                                                                                                                           {
  & & \node(root-syntax-tree-5){$\slabs{\avar}$}; \\
  & & \node(0-syntax-tree-5){$\slabs{f}$}; \\ 
  & & \node(00-syntax-tree-5){$\sslapp$}; \\
  & \node(000-syntax-tree-5){$\sslapp$}; \\
  \node(0000-syntax-tree-5){$f$}; & & \node(helper1-syntax-tree-5)[draw=none]{}; \\   
  & & \node(helper2-syntax-tree-5)[draw=none]{}; & & & & & \node(001-syntax-tree-5){$\avar$};\\
};    
\draw[-,thick](root-syntax-tree-5) to (0-syntax-tree-5);
\draw[-](0-syntax-tree-5) to (00-syntax-tree-5);
\draw[-](00-syntax-tree-5) to (000-syntax-tree-5);
\draw[-](000-syntax-tree-5) to (0000-syntax-tree-5);
\draw[-](00-syntax-tree-5) to (001-syntax-tree-5);
\draw[->](000-syntax-tree-5) to[out=-50,in=50,distance=1.75cm] 
                  (00-syntax-tree-5); 
%
\draw[-,dashed,thick,red]
  (0000-syntax-tree-5) -- ($ (helper1-syntax-tree-5) + (2.65cm,0cm) $)  %($ (helper1-syntax-tree-5) + (1.1cm,0cm) $)
         -- ($ (0-syntax-tree-5) + (2.65cm,0cm) $)        %($ (0-syntax-tree-5) + (1.1cm,0cm) $)
         -- (0-syntax-tree-5);               
%                                                
\draw[-,dashed,thick,red]
  (001-syntax-tree-5) -- ($ (helper2-syntax-tree-5) + (3.2cm,0cm) $)
        -- ($ (root-syntax-tree-5) + (3.2cm,0cm) $)
        -- (root-syntax-tree-5);
% 
\end{pgfonlayer}{graph}                  
 

\begin{pgfonlayer}{innerscope}    
  \draw[draw=none,fill=grey!27]
    (0000-syntax-tree-5) -- ($ (helper1-syntax-tree-5) + (2.65cm,0cm) $)  %($ (helper1-syntax-tree-5) + (1.1cm,0cm) $)
           -- ($ (0-syntax-tree-5)       + (2.65cm,0cm) $)        %($ (0-syntax-tree-5) + (1.1cm,0cm) $)\
           -- ($ (0-syntax-tree-5)       + (-2.65cm,0cm) $)
           -- ($ (helper1-syntax-tree-5) + (-2.65cm,0cm) $)
           -- (0000-syntax-tree-5);           
\end{pgfonlayer}{innerscope}
                                  

\begin{pgfonlayer}{outerscope}                                 
  \draw[draw=none,fill=grey!12]
    (001-syntax-tree-5) -- ($ (helper2-syntax-tree-5) + (3.2cm,0cm) $)
          -- ($ (root-syntax-tree-5) + (3.2cm,0cm) $)
          -- ($ (root-syntax-tree-5) + (-3.2cm,0cm) $)
          -- ($ (helper2-syntax-tree-5) + (-3.2cm,0cm) $)
          -- (001-syntax-tree-5);
\end{pgfonlayer}                                        

    
\begin{pgfonlayer}{caption}  
  \path[draw=none] (root-syntax-tree-5) -- ($ (root-syntax-tree-5) + (0cm,-4.7cm) $) node{syntax tree (+ recursive backlink};
  \path[draw=none] (root-syntax-tree-5) -- ($ (root-syntax-tree-5) + (0cm,-5.2cm) $) node{+ scope sets, \textcolor{red}{+ binding links})};
\end{pgfonlayer}
  
  
\begin{pgfonlayer}{boundingbox}  
  \path[thick,dotted,%draw,
                     use as bounding box]
       ($ (root-syntax-tree-5.north) + (-3.5cm,0.15cm) $)
    -- ($ (root-syntax-tree-5.north) + (-3.5cm,-5.6cm) $)
    -- ($ (root-syntax-tree-5.north) + (+3.5cm,-5.6cm) $)
    -- ($ (root-syntax-tree-5.north) + (+3.5cm,0.15cm) $)
    -- ($ (root-syntax-tree-5.north) + (-3.5cm,0.15cm) $);
\end{pgfonlayer}
